Lynx: An Open Source Hallucination Evaluation Model

Retrieval Augmented Generation (RAG) techniques aim to mitigate hallucinations in Large Language Models (LLMs). However, LLMs can still produce information that is unsupported or contradictory to the retrieved contexts. We introduce LYNX, a SOTA hallucination detection LLM that is capable of advanced reasoning on challenging real-world hallucination scenarios. To evaluate LYNX, we present HaluBench, a comprehensive hallucination evaluation benchmark, consisting of 15k samples sourced from various real-world domains. Our experiment results show that LYNX outperforms GPT-4o, Claude-3-Sonnet, and closed and open-source LLM-as-a-judge models on HaluBench. We release LYNX, HaluBench and our evaluation code for public access.

==> tables/table1.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage[normalem]{ulem}
% % \useunder{\uline}{\ul}{}
% \begin{table*}[htbp]
% \small
% \centering
% \begin{tabular}{l|cccccc|c}
% \hline\hline
% & \begin{tabular}[c]{@{}l@{}}Numerical reasoning:\\ multiple financial\\ statements\end{tabular} & \begin{tabular}[c]{@{}l@{}}Numerical reasoning:\\ single financial\\ statement\end{tabular} & \begin{tabular}[c]{@{}l@{}}Information\\ extraction\end{tabular} & \begin{tabular}[c]{@{}l@{}}Overall \%\\ correct\end{tabular} \\
% \hline\hline
% \begin{tabular}[c]{@{}l@{}}GPT4\\ No context\end{tabular} & 0\% & 3\% & 0\% & \textbf{1\%} \\
% \begin{tabular}[c]{@{}l@{}}GPT4\\ All docs in\\ one vector store\end{tabular} & 13\% & 21\% & 21\% & \textbf{18\%} \\
% \begin{tabular}[c]{@{}l@{}}GPT4\\ One doc per\\ vector store\end{tabular} & 13\% & 39\% & 29\% & \textbf{26\%} \\
% \begin{tabular}[c]{@{}l@{}}Llama2\\ One doc per\\ vector store\end{tabular} & 15\% & 12\% & 29\% & \textbf{18\%} \\
% \begin{tabular}[c]{@{}l@{}}GPT4\\ Evidence \\ strings\end{tabular} & \textbf{51\%} & \textbf{73\%} & \textbf{86\%} & \ul{\textbf{68\%}} \\
% \begin{tabular}[c]{@{}l@{}}Anthropic\\ Long\\ context\end{tabular} & 23\% & 42\% & 57\% & \textbf{39\%} \\
% \textbf{\begin{tabular}[c]{@{}l@{}}\% of\\ type\\ correct\end{tabular}} & \textbf{19\%} & \textbf{32\%} & \ul{\textbf{37\%}} & \\
% \hline\hline
% \end{tabular}
% \label{tab:metrics_performance}
% \end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% SECOND IMPLEMENTATION %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[htbp]
\small
\centering
\begin{tabular}{l|cccccc|c}

& \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}GPT4\\ No context\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}GPT4\\ All docs in\\ one vector store\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}GPT4\\ One doc per\\ vector store\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Llama2\\ One doc per\\ vector store\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}GPT4\\ Evidence \\ strings\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Anthropic\\ Long\\ context\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\% of\\ type\\ correct\end{tabular}} \\
\hline
\hline
\begin{tabular}[c]{@{}l@{}}Numerical reasoning:\\ multiple financial\\ statements\end{tabular} & 0\%                                                                           & 13\%                                                                                              & 13\%                                                                                          & 15\%                                                                                            & \textbf{51\%}                                                                          & 23\%                                                                                   & \textbf{19\%}                                                           \\
\hline
\begin{tabular}[c]{@{}l@{}}Numerical reasoning:\\ single financial\\ statement\end{tabular}    & 3\%                                                                           & 21\%                                                                                              & 39\%                                                                                          & 12\%                                                                                            & \textbf{73\%}                                                                          & 42\%                                                                                   & \textbf{32\%}                                                           \\
\hline
\begin{tabular}[c]{@{}l@{}}Information\\ extraction\end{tabular}                               & 0\%                                                                           & 21\%                                                                                              & 29\%                                                                                          & 29\%                                                                                            & \textbf{86\%}                                                                          & 57\%                                                                                   & {\ul \textbf{37\%}}                                                     \\
\hline
\textbf{\begin{tabular}[c]{@{}l@{}}Overall \%\\ correct\end{tabular}}                          & \textbf{1\%}                                                                  & \textbf{18\%}                                                                                     & \textbf{26\%}                                                                                 & \textbf{18\%}                                                                                   & {\ul \textbf{68\%}}                                                                    & \textbf{39\%}                                                                          &                                                                         \\ 
\end{tabular}
\caption{Model performance on the three types of metrics-generated questions}
\label{tab: metrics_performance}
\end{table*}

==> tables/table2.tex <==


\begin{table*}[t]
\vspace{-5mm}
\small
\centering
\begin{tabular}{l|l|ccc|c}
\toprule
\multirow{2}{*}{\parbox{2cm}{\centering\textbf{Company}}} & \multirow{2}{*}{\parbox{4cm}{\centering\textbf{GICS Sector}}} & \multirow{2}{*}{\parbox{1.6cm}{\centering\textbf{Metrics-generated}}} & \multirow{2}{*}{\parbox{1.6cm}{\centering\textbf{Domain-relevant}}}  & \multirow{2}{*}{\parbox{1.6cm}{\centering\textbf{Novel generated}}} & \multirow{2}{*}{\parbox{1.6cm}{\centering\textbf{Total}}} \\
 & & & & \\
\midrule
\rule{0pt}{4pt}% Adjust the height of the space here
3M & Industrials & 269 & 25 & 36 & 330 \\
Boeing & Industrials & 248 & 25 & 47 & 320 \\
CVS Health & Health Care & 253 & 25 & 23 & 301 \\
Coca-Cola & Consumer Staples  & 239 & 25 & 25 & 289 \\
MGM Resorts & Consumer Discretionary & 196 & 25 & 26 & 247 \\
Netflix & Communication Services & 242 & 25 & 25 & 292 \\
Pfizer & Health Care & 156 & 25 & 58 & 239 \\
Salesforce & Information Technology & 0 & 25 & 25 & 50 \\
Ulta Beauty & Consumer Discretionary & 0 & 25 & 25 & 50 \\
Verizon & Communication Services & 272 & 25 & 50 & 347 \\
\bottomrule
%\textbf{Total} & & \textbf{7,983} & \textbf{925} & \textbf{1,323} & \textbf{10,231} \\
\end{tabular}
\caption{Selection of 10 companies in \textsc{FinanceBench}}
\label{tab:dataset_summary}
\end{table*}

==> tables/table3.tex <==
\begin{table}[]
\begin{tabular}{l|cc|c}
\toprule
                      & \textbf{GPT-4}                                         & \textbf{Llama2}                                        & \textbf{Average}                                       \\
\midrule
\textbf{Correct}      & \begin{tabular}[c]{@{}c@{}}4,584\\ (45\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}3,595\\ (35\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}4,090\\ (40\%)\end{tabular} \\
\midrule
\textbf{Incorrect}    & \begin{tabular}[c]{@{}c@{}}976\\ (10\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}6,156\\ (60\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}3,566\\ (35\%)\end{tabular} \\
\midrule
\textbf{Refusal}      & \begin{tabular}[c]{@{}c@{}}4,671\\ (46\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}480\\ (5\%)\end{tabular}    & \begin{tabular}[c]{@{}c@{}}2,576\\ (25\%)\end{tabular} \\
\midrule
\textbf{Failure rate} & 56\%                                                   & 65\%                                                   & 60\% \\
\bottomrule
\end{tabular}
\caption{Performance of two models on the full 10,231 entry dataset in \textsc{FinanceBench}, evaluated automatically.}
\label{tab:eval_performance}
\end{table}

==> tables/table4.tex <==

\begin{table*}[ht]
\small
\centering
\begin{tabular}{ll|ccc|c}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Configuration}} & \multirow{2}{*}{\textbf{Correct answer}} & \multirow{2}{*}{\textbf{Incorrect answer}} & \multirow{2}{*}{\textbf{Failed to answer}} & \multirow{2}{*}{\textbf{Total}} \\
&&&& \\ % This empty row is necessary for the multirow cells to align properly
\midrule
\multirow{2}{*}{\texttt{GPT-4-Turbo}} & Closed Book    & \multirow{2}{*}{14 (9\%)}      & \multirow{2}{*}{5 (3\%)}  & \multirow{2}{*}{126 (88\%)}  & \multirow{2}{*}{150}            \\
& (on its own) &  &   & &             \\
\midrule
 % \multirow{2}{*}{Llama2}&Shared Vector Store & 29 (19\%)   & 104 (70\%)   & 17 (11\%) & 150  \\
 %    &(one store for all filings) \\
\multirow{2}{*}{\texttt{Llama2}} & Shared Vector Store & \multirow{2}{*}{29 (19\%)}   & \multirow{2}{*}{104 (70\%)}   & \multirow{2}{*}{17 (11\%)} & \multirow{2}{*}{150  }          \\
 & (one store for all filings) &  &   & &             \\
%\midrule
\multirow{2}{*}{\texttt{GPT-4-Turbo}} & Shared Vector Store & \multirow{2}{*}{29 (19\%)}  & \multirow{2}{*}{20 (13\%)} & \multirow{2}{*}{101 (68\%)} & \multirow{2}{*}{150}            \\
& (one store for all filings) &  &   & &             \\
\midrule
\multirow{2}{*}{\texttt{Llama2}} & Single Vector Store & \multirow{2}{*}{62 (41\%) }  & \multirow{2}{*}{81 (54\%) }   & \multirow{2}{*}{7 (5\%)} & \multirow{2}{*}{150 }           \\
& (one store for each filing) &  &   & &             \\
%\midrule
%GPT-4 with evidence pages
\multirow{2}{*}{\texttt{GPT-4-Turbo}} & Single Vector Store & \multirow{2}{*}{75 (50\%)} & \multirow{2}{*}{17 (11\%)} & \multirow{2}{*}{58 (39\%)}  & \multirow{2}{*}{150  }         \\
& (one store for each filing) &  &   & &             \\
\midrule
\multirow{2}{*}{\texttt{Claude2}} & Long Context & \multirow{2}{*}{114 (76\%)}   & \multirow{2}{*}{32 (21\%)} & \multirow{2}{*}{4 (3\%)} & \multirow{2}{*}{150 }           \\
& (filing in context) &  &   & &             \\
%\midrule
\multirow{2}{*}{\texttt{GPT-4-Turbo}} & Long Context & \multirow{2}{*}{118 (79\%)}   & \multirow{2}{*}{26 (17\%)} & \multirow{2}{*}{6 (4\%)}  & \multirow{2}{*}{150 }           \\
& (filing in context) &  &   & &             \\
\midrule
\multirow{2}{*}{\texttt{GPT-4-Turbo}} & Oracle& \multirow{2}{*}{128 (85\%)}  &\multirow{2}{*}{ 22 (15\%)} & \multirow{2}{*}{0 (0\%)}  &\multirow{2}{*}{ 150 }           \\
& (access to evidence pages) &  &   & &             \\
\midrule
% \textbf{Total} & 733 & 407 & 648 & 1,788 \
\multirow{2}{*}{\textbf{Total}} & & \multirow{2}{*}{569 (47\%)} & \multirow{2}{*}{307 (26\%)} & \multirow{2}{*}{324 (27\%)} & \multirow{2}{*}{1200} \\ % Empty cell for the second line of the total row
&&&& \\ % Empty row for the second line of the total row\
\bottomrule
\end{tabular}
\caption{Model performance of 8 model configurations on \textsc{FinanceBench} human eval sample (n=150).}
\label{tab:model_performance_table}
\end{table*}

==> tables/table5.tex <==

\begin{table*}[ht]
\centering
\begin{tabular}{l|c|c|l|c}
\toprule
\textbf{Company}     & \textbf{Symbol} & \textbf{Market cap} & \textbf{GICS Sector}   & \textbf{S\&P 500} \\
\midrule
3M                   & MMM             & \$48.5 billion      & Industrials            & Yes               \\
AES Corporation      & AES             & \$8.44 billion      & Utilities              & Yes               \\
Amcor                & AMCR            & \$12.92 billion     & Materials              & Yes               \\
AMD                  & AMD             & \$166.27 billion    & Information Technology & Yes               \\
Activision Blizzard  & ATVI            & \$73.7 billion      & Communication Services & Yes               \\
Adobe                & ADBE            & \$235.14 billion    & Information Technology & Yes               \\
American Express     & AXP             & \$108.33 billion    & Financials             & Yes               \\
American Water Works & AWK             & \$23.11 billion     & Utilities              & Yes               \\
Apple                & AAPL            & \$2730 billion      & Information Technology & Yes               \\
Best Buy             & BBY             & \$14.72 billion     & Consumer Discretionary & Yes               \\
Boeing               & BA              & \$112.37 billion    & Industrials            & Yes               \\
CVS Health           & CVS             & \$89.59 billion     & Health Care            & Yes               \\
Coca-Cola            & KO              & \$226.51 billion    & Consumer Staples       & Yes               \\
Corning              & GLW             & \$25.32 billion     & Information Technology & Yes               \\
Costco               & COST            & \$252.18 billion    & Consumer Staples       & Yes               \\
eBay                 & EBAY            & \$22.68 billion     & Consumer Discretionary & Yes               \\
FedEx                & FDX             & \$65.16 billion     & Industrials            & Yes               \\
Foot Locker          & FL              & \$1.79 billion      & Consumer Discretionary & No                \\
General Mills        & GIS             & \$36.25 billion     & Consumer Staples       & Yes               \\
Intel                & INTC            & \$150.31 billion    & Information Technology & Yes               \\
JPMorgan             & JPM             & \$415.28 billion    & Financials             & Yes               \\
Johnson  Johnson     & JNJ             & \$378.4 billion     & Health Care            & Yes               \\
Lockheed Martin      & LMT             & \$100.07 billion    & Industrials            & Yes               \\
MGM Resorts          & MGM             & \$12.21 billion     & Consumer Discretionary & Yes               \\
McDonalds            & MCD             & \$183.82 billion    & Consumer Discretionary & Yes               \\
Microsoft            & MSFT            & \$2370 billion      & Information Technology & Yes               \\
Nike                 & NKE             & \$146.56 billion    & Consumer Discretionary & Yes               \\
Netflix              & NFLX            & \$165.11 billion    & Communication Services & Yes               \\
Oracle               & ORCL            & \$296.81 billion    & Information Technology & Yes               \\
PGE Corporation      & PCG             & \$39.41 billion     & Utilities              & Yes               \\
Paypal               & PYPL            & \$63.12 billion     & Financials             & Yes               \\
PepsiCo              & PEP             & \$220.39 billion    & Consumer Staples       & Yes               \\
Pfizer               & PFE             & \$188.97 billion    & Health Care            & Yes               \\
Salesforce           & CRM             & \$196.56 billion    & Information Technology & Yes               \\
Ulta Beauty          & ULTA            & \$19.14 billion     & Consumer Discretionary & Yes               \\
Verizon              & VZ              & \$133.77 billion    & Communication Services & Yes               \\
Walmart              & WMT             & \$428.17 billion    & Consumer Staples       & Yes               \\
Block                & SQ              & \$26.8 billion      & Information Technology & No                \\
Amazon               & AMZN            & \$1325 billion      & Consumer Discretionary & Yes               \\
Kraft Heinz          & KHC             & \$33.47 billion     & Consumer Staples       & Yes    \\           
\bottomrule
\end{tabular}
\caption{Summary of companies that appear in \textsc{FinanceBench}}
\label{tab:company_summary}
\end{table*}
